IncBL: Incremental Bug Localization

Numerous efforts have been invested in improving the effectiveness of bug localization techniques, whereas little attention is paid to making these tools run more efficiently in continuously evolving software repositories. This paper first analyzes the information retrieval model behind a classic bug localization tool, BugLocator, and builds a mathematical foundation illustrating that the model can be updated incrementally when codebase or bug reports evolve. Then, we present IncBL, a tool for Incremental Bug Localization in evolving software repositories. IncBL is evaluated on the Bugzbook dataset, and the results show that IncBL can significantly reduce the running time by 77.79% on average compared with the re-computing the model, while maintaining the same level of accuracy. We also implement IncBL as a Github App that can be easily integrated into open-source projects on GitHub. Users can deploy and use IncBL locally as well. The demo video for IncBL can be viewed at https://youtu.be/G4gMuvlJSb0, and the source code can be found at https://github.com/soarsmu/IncBL.

==> Makefile <==
# Makefile for a latex paper
LATEX = TEXINPUTS=$(TEXINPUTS):packages pdflatex
PAPER = IncBL

all: $(PAPER).pdf

#I don't have gs and don't want to see errors
quick: $(wildcard *.tex) $(wildcard sections/*.tex) $(wildcard *.bib)
	$(LATEX) $(PAPER).tex </dev/null
	bibtex $(PAPER)
	$(LATEX) $(PAPER).tex </dev/null
	$(LATEX) $(PAPER).tex </dev/null

# Run once, then re-run until it's happy
# Input redirected from /dev/null is like hitting ^C at first error
$(PAPER).pdf: $(wildcard *.tex) $(wildcard sections/*.tex) $(wildcard *.bib)
	$(LATEX) $(PAPER).tex </dev/null
	bibtex $(PAPER)
	$(LATEX) $(PAPER).tex </dev/null
	$(LATEX) $(PAPER).tex </dev/null
	gs -q -dNOPAUSE -dBATCH -dPDFSETTINGS=/prepress -dEmbedAllFonts=true \
       -dDownsampleColorImages=false -dAutoFilterColorImages=false \
       -dColorImageFilter=/FlateEncode -sDEVICE=pdfwrite -sOutputFile=$(PAPER)-embed.pdf \
       $(PAPER).pdf
	mv $(PAPER)-embed.pdf $(PAPER).pdf

Figures: 
	
.PHONY: pdf print
print: $(PAPER).pdf
	open $(PAPER).pdf

clean:
	rm -f *.aux *.log $(PAPER).pdf *.blg *.bbl *.lof *.lot *.toc *.fls *.out *.fdb_latexmk *.cut *~


==> sections/limitation.tex <==
\section{Limitation}
\label{sec:limit}
Whether a bug localization tool can be made incremental highly depends on how they model the localization process. The incremental design we propose can be migrated to other IRBL approaches like BLUiR \cite{BLUiR}. However, it is harder to incremental update neural-IR tools that may require retraining when repositories change.
